Human-Centered Autonomy for UAS Target Search

Current methods of deploying robots that operate in dynamic, uncertain environments, such as Uncrewed Aerial Systems in search \& rescue missions, require nearly continuous human supervision for vehicle guidance and operation. These methods do not consider high-level mission context resulting in cumbersome manual operation or inefficient exhaustive search patterns. We present a human-centered autonomous framework that infers geospatial mission context through dynamic feature sets, which then guides a probabilistic target search planner. Operators provide a set of diverse inputs, including priority definition, spatial semantic information about ad-hoc geographical areas, and reference waypoints, which are probabilistically fused with geographical database information and condensed into a geospatial distribution representing an operator's preferences over an area. An online, POMDP-based planner, optimized for target searching, is augmented with this reward map to generate an operator-constrained policy. Our results, simulated based on input from five professional rescuers, display effective task mental model alignment, 18\% more victim finds, and 15 times more efficient guidance plans then current operational methods.

==> background_old.tex <==
% Background Section Source File
% The ability of UAS to rapidly cover large areas at an affordable cost to agencies makes their deployment increasingly invaluable. However, while learning to fly today's aircraft can be accomplished in an afternoon, integrating the platform within a developing incident relies on years of experience and training. 

\subsection{Problem Statement}
%Search and rescue incidents are characterized by the pursuit, localization, and extraction of one or more people in distress in diverse environments. 

A search operation takes place over a larger state space, $S\subseteq \mathbb{R}^f$, representing $f$ mission influencing factors, including static (geography) or dynamic (team locations) variables. The operator acts as a means of fusing the contextual and environmental aspects of an evolving operation. They provide a set of inputs, $\mathcal{I}$, that correspond to their preferences over sections to search. $\mathcal{I}$ must be interpreted along with vehicle performance metrics such as limited battery life, to generate a time optimal guidance policy, $\pi$, which outputs incremental waypoints, $\mathcal{W}\in \mathbb{R}^2$, to effectively search an area. The aircraft can perform its internal navigation and control to efficiently follow $\mathcal{W}$ \zs{I think this should be a feedback policy on observations rather than waypoints} while looking for infrared hotpots or visual clues as to a static victim's location. This detection can be accomplished through computer vision or rely on the operator, however this is outside the scope of this work.

We motivate our work with a hypothetical incident, derived from real-life scenarios, without loss of generality. In this scenario, a middle-aged man, a frequent fly-fisherman, was reported missing by his wife after he failed to return from a daytime trip to the Walker Ranch Open Space in Boulder County, CO. The victim's vehicle was found at the southern trailhead. The first arriving unit includes a UAS team, which are tasked with performing a preliminary search of the area. 

With this knowledge, an officer directing operations gains awareness of the victim's physical condition, potential equipment, last-know-point, and behavior. These factors of their evolving mental model are then grounded in the mission area, which informs the resulting search methods. While searching for our lost fisherman, minimizing the operator's oversight of the vehicle through minimal inputs allows them to move across the environment, remain closer to ground teams, change vehicle line-of-sight, and maintain situational awareness, all of which should result in a faster rescue time. 

\zs{I think we should add a preview of the *key features* of our solution (i.e. sketch interface, RINAO to process $I$ and $HIPPO$ to determine the policy) here and point to the figure. EDIT: As per our discussion, this can go in the intro after defining I}

% \begin{problem}[human in the loop]

% \zl{General Human-in-the-loop target search problem}

% \end{problem}

\subsection{Related Work}
Rescuers leverage years of training, operational experience, local knowledge, and incident information to form their mental model of an evolving operation, which they then use to inform a provided task to subordinate human or robot teammates \cite{rouse_looking_1986}. Robots can interpret mental models in multiple ways \cite{tabrez_survey_2020} and robotic teams that use shared mental models have been shown to improve their performance \cite{gervits_toward_2020}. However, many mental model frameworks rely on static, pre-defined architectures shared by all actors \cite{scheutz_framework_2017},\cite{albrecht_autonomous_2018}. Our research decouples the interpretation of the operator's $\mathcal{I}$ with the vehicle planning and execution, enabling a flexible `plug-and-play' approach centered on operator direction, while accommodating diverse underlying autonomous architectures.

In practice, autonomous robots have been successfully directed by their operators using other human-autonomy interaction methods. The approach in \cite{jamieson_active_2020} uses a POMDP to fuse the operator's inputs with the planning \& execution for robot search tasks, although their approach severely limits the complexity of operator inputs. The approach in \cite{arora_multi-modal_2019} uses Bayesian priors on geological knowledge to effectively define operator preferences for planning and execution, but lacks an intuitive interface for non-engineers to craft/update preferences in real-time. The direction realized through sets of `plays' found in \cite{miller_delegation_2014}, breaks down a complex mission into smaller tasks, but additionally requires a homogeneous autonomy architecture. While operators can modify each task individually, there is no systematic way to define operator preferences across a whole mission set.

Inverse Reinforcement Learning (IRL) problems reflect our efforts to learn a user's reward function by extracting context from inputs. However, whereas IRL relies on observed expected behaviour, such as reference trajectories, to directly infer reward functions \cite{arora_survey_2021}, we infer feature values by fusing multi-modal inputs and readily available geographic database information. Operators may not provide trajectories that optimally account for aircraft performance, and so while operators could draw multiple reference trajectories to inform an IRL solution, learning low-level trajectory information is not as efficient as using a richer set of inputs to understand higher-level preferences in the context of search and rescue. Applying the learned reward distribution on top of a planner allows its baseline performance to be augmented by end user expertise, addressing the challenges found with rewards designed by engineers \cite{hadfield-menell_inverse_2017},\cite{booth_perils_2023}. 


Leveraging autonomy in search tasks can significantly reduce the burden on rescue personnel. Kingston et al. \cite{kingston2016automated} introduce an intermediate level of autonomy by providing the operator with parametrized tasks and common UAS search/surveillance patterns \nisarcomm{(e.g. lawnmower)}. These approaches can be quite effective and are often used by U.S. maritime search and rescue personnel \cite{thomas2013us}. However, these approaches do not directly model the target location uncertainty. Search tasks require dynamic decision making using realtime observations. Bourgault et al. \cite{bourgault2006optimal} adopts a Bayesian approach and models the target location using a non-uniform prior distribution. Obtaining an accurate and informed prior over the target location is often challenging. Our approach uses a uniform distribution and makes no assumptions about the target's initial location. We do this by leveraging POMDPs.  

POMDPs can efficiently capture the aleatoric and epistemic uncertainty of a system \cite{kochenderfer2022algorithms}, making them a natural candidate for modeling search tasks. We use a POMDP to model expert-provided domain knowledge as dynamic reward and allow observations to inform and shape the target belief over time. This way, we can flexibly express domain knowledge and operator preferences as a measure of utility in search objectives. 


Several works explore the use of POMDPs for object search in cluttered environments \cite{zheng2021multi, wandzel2019multi, xiao2019online} with object segmentation and classification. Wandzel et al. incorporate structured natural language commands into factored POMDP belief updates. Xiao et al. leverage grasping robots to aid in decluttering the search space. These approaches are able to perform well in smaller search environments. Our approach investigates larger target search spaces commonly encountered in search and rescue and flexibly integrates human expert information through not only semantic language but through expressive sketches. 

POMDPs have also been used to model target search. Baker et al. \cite{baker2016planning} leverage POMDPs for search and rescue, incorporating available emergency data sources such as crowd reports or cell signals into the observation models. Our approach delegates external target/domain knowledge to the operator thereby reducing modeling complexity in the POMDP and allowing the planner to search deeper. Additionally, our approach does not rely on any on-person target data and instead allows for \textit{human-on-the-loop} collaboration, where the human can provide inputs at any time during the search but is not a critical component in the autonomy loop. 

\zl{summarize main contribution/approach here}

% \nisarcomm{careful about the claim you are making here: are these issues completely avoided for all kinds of possible tasks? still need to make model to represent these on an arbitrary scale? or are only some specific aspects that are most relevant to UAS SAR information gathering problem mitigated? which ones and how/why exactly?}
%\nisarcomm{somewhat begs the question: why not have SAR UAS operators provide example trajectories and then use IRL?} 

